Scaling Laws for Hyperparameter Optimization

Hyperparameter optimization is an important subfield of machine learning that focuses on tuning the hyperparameters of a chosen algorithm to achieve peak performance. Recently, there has been a stream of methods that tackle the issue of hyperparameter optimization, however, most of the methods do not exploit the dominant power law nature of learning curves for Bayesian optimization. In this work, we propose Deep Power Laws (DPL), an ensemble of neural network models conditioned to yield predictions that follow a power-law scaling pattern. Our method dynamically decides which configurations to pause and train incrementally by making use of gray-box evaluations. We compare our method against 7 state-of-the-art competitors on 3 benchmarks related to tabular, image, and NLP datasets covering 59 diverse tasks. Our method achieves the best results across all benchmarks by obtaining the best any-time results compared to all competitors.

==> Plots/cifar10_different_schedulers.tex <==
\begin{figure}[!t]
    \centering 
    %\medskip
    \includegraphics[width=\textwidth]{Figures/surrogate_different_schedulers.pdf}
    \caption[Predicting the target curves with DPL for different learning rate schedulers]{Comparing $ f(\lambda=0.45, b)$ and $\hat f(\lambda=0.45, b)$ across budgets $b$ for different learning rate schedulers.}
    \label{fig:cifa10_different_schedulers}
    %\vspace{-0.5cm}
\end{figure}


==> Plots/cifar10_motivation.tex <==
\begin{wrapfigure}{!hr}{0.5\textwidth}
    \centering 
\includegraphics[width=0.4\textwidth]{Figures/cifar10_motivational_example.pdf}
    \caption[Predicting and uncertainty modelling of the power law surrogate.]{The power law predictions and uncertainty estimations on the CIFAR10 1-D search space. \textbf{Top:} The real performance $f(\lambda, b=50)$ in black and our surrogate $\hat f(\lambda, b=50)$ in red across configurations $\lambda$ on the maximum budget $b=50$. \textbf{Bottom:} Comparing $ f(\lambda=0.45, b)$ and $\hat f(\lambda=0.45, b)$ across budgets $b$.}
    \label{fig:cifa10_power_law_modelling}
    \vspace{-0.5cm}
\end{wrapfigure}


==> Plots/explored_configuration_distributions.tex <==
\begin{figure}[htbp]
    \centering 
    %\medskip
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=\textwidth]{Figures/config_distribution_lcbench.pdf}
      %\caption{Gain over the number of examples}
      %\label{fig:1}
    \end{subfigure}%\hfil % <-- added
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=\textwidth]{Figures/config_distribution_taskset.pdf}
      %\label{fig:2}
    \end{subfigure}%\hfil % <-- added
    \begin{subfigure}{0.33\textwidth}
      \includegraphics[width=\textwidth]{Figures/config_distribution_pd1.pdf}
      %\label{fig:2}
    \end{subfigure}%\hfil % <-- added
    \caption[The configuration distributions for all baselines.]{The distributions of unique explored hyperparameter configurations for all methods considered over all datasets in every corresponding baseline.}
    \label{fig:power_law_explored_configurations}
    %\vspace{-0.5cm}
\end{figure}


==> Plots/power_law_modelling_cifar10.tex <==
\begin{figure}[htbp]
    \centering 
    \includegraphics[width=\textwidth]{Figures/power_law_modelling.pdf}
    \caption[Predicting and uncertainty modelling of the power law surrogate.]{The power law predictions and uncertainty on:  \textbf{Left:} Across different budgets for the same hyperparameter configuration that was observed partially. \textbf{Right:} The highest budget across different hyperparameter configurations (dropout rates).}
    \label{fig:cifa10_power_law_modelling}
    %\vspace{-0.5cm}
\end{figure}


==> Plots/top_configs_dpl_correlations.tex <==
\begin{SCfigure}
    \centering
    \includegraphics[width=0.65\textwidth]{Figures/top_configs_model_correlations.pdf}
    \caption[The correlation of DPLs and neural networks for the top 100 configs.]{The distribution of correlations for the top-100 configurations of the neural network and the DPL for different fractions of observed learning curves across datasets.
    \vspace{1.4cm}}
    \label{fig:conditioned_pl_correlations_top100}
\end{SCfigure}

==> Tables/power_law_times.tex <==
\begin{wraptable}{!tr}{0.5\textwidth}
%\begin{table}
 \centering
 \footnotesize
 \begin{adjustbox}{width=0.4\textwidth}{
 \begin{tabular}{@{}ccc@{}}
  \toprule
  \textbf{Benchmark} & \textbf{Time (seconds)} & \textbf{Batch Size} \\ \midrule
  LCBench & 0.034 & 32 \\
  TaskSet & 0.034 & 32 \\
  PD1 & 	8.08e-06 & 32 \\
  \bottomrule 
 \end{tabular}
 }\end{adjustbox}
 \caption{\label{app:power_law_times} DPL overhead to fit a batch of examples on the datasets of different benchmarks.}
 \vspace{-0.5cm}
%\end{table}
\end{wraptable}

==> Text/9-limitations.tex <==
\section{Limitations}

Our proposed ensemble of power law functions sets the new state-of-the-art in gray-box HPO and highlights the efficiency of modeling learning curves with a power law assumption. However, contrary to the common perception, we experienced that the uncertainty estimation arising from the Deep Ensemble approach~\citep{Lakshminarayanan2017} is suboptimal compared to standard BO surrogates such as Gaussian Processes. In the future, we plan to investigate the combination of power laws with Gaussian Processes.

%However, we believe that further research is needed to calibrate the power law model for the beginning and the end parts of the learning curves. 
%Recent work highlighted that the error rate at very small budgets (e.g. after a few mini-batches) is not a power law~\citep{Rosenfeld2021}. 

 %In addition, having to train an ensemble has additional computational costs, due to the necessity of training multiple power law models. 


